Gravitational-wave astronomy with a physical calibration model

We carry out astrophysical inference for compact binary merger events in LIGO-Virgo's first gravitational-wave transient catalog (GWTC-1) using a physically motivated calibration model. We demonstrate that importance sampling can be used to reduce the cost of what would otherwise be a computationally challenging analysis. We show that including the physical estimate for the calibration error distribution has negligible impact on the inference of parameters for the events in GWTC-1. Studying a simulated signal with matched filter signal-to-noise ratio $\text{SNR}=200$, we project that a calibration error estimate typical of GWTC-1 is likely to be negligible for the current generation of gravitational-wave detectors. We argue that other sources of systematic error---from waveforms, prior distributions, and noise modelling---are likely to be more important. Finally, using the events in GWTC-1 as standard sirens, we infer an astrophysically-informed improvement on the estimate of the calibration error in the LIGO interferometers.

==> other_plots.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.48\linewidth]{figs/GW151012_intrinsic}
    \includegraphics[width=0.48\linewidth]{figs/GW151012_extrinsic}
    \includegraphics[width=\linewidth]{figs/GW151012_calibration}
    \caption{GW151012}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.48\linewidth]{figs/GW151226_intrinsic}
    \includegraphics[width=0.48\linewidth]{figs/GW151226_extrinsic}
    \includegraphics[width=\linewidth]{figs/GW151226_calibration}
    \caption{GW151226}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.48\linewidth]{figs/GW170104_intrinsic}
    \includegraphics[width=0.48\linewidth]{figs/GW170104_extrinsic}
    \includegraphics[width=\linewidth]{figs/GW170104_calibration}
    \caption{GW170104}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.48\linewidth]{figs/GW170608_intrinsic}
    \includegraphics[width=0.48\linewidth]{figs/GW170608_extrinsic}
    \includegraphics[width=\linewidth]{figs/GW170608_calibration}
    \caption{
    GW170608. 
    \colm{Ask calibration team about whether this event is interesting due to calibration work taking place at the time of this event. Note also that the deviation in calibration is more clearly visible in H1 than in L1. Please add the efficiency plot.} 
    }
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.48\linewidth]{figs/GW170729_intrinsic}
    \includegraphics[width=0.48\linewidth]{figs/GW170729_extrinsic}
    \includegraphics[width=\linewidth]{figs/GW170729_calibration}
    \caption{GW170729}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.48\linewidth]{figs/GW170809_intrinsic}
    \includegraphics[width=0.48\linewidth]{figs/GW170809_extrinsic}
    \includegraphics[width=\linewidth]{figs/GW170809_calibration}
    \caption{GW170809}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.48\linewidth]{figs/GW170814_intrinsic}
    \includegraphics[width=0.48\linewidth]{figs/GW170814_extrinsic}
    \includegraphics[width=\linewidth]{figs/GW170814_calibration}
    \caption{GW170814}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.48\linewidth]{figs/GW170817_intrinsic}
    \includegraphics[width=0.48\linewidth]{figs/GW170817_extrinsic}
    \includegraphics[width=\linewidth]{figs/GW170817_calibration}
    \caption{GW170817}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.48\linewidth]{figs/GW170818_intrinsic}
    \includegraphics[width=0.48\linewidth]{figs/GW170818_extrinsic}
    \includegraphics[width=\linewidth]{figs/GW170818_calibration}
    \caption{GW170818}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.48\linewidth]{figs/GW170823_intrinsic}
    \includegraphics[width=0.48\linewidth]{figs/GW170823_extrinsic}
    \includegraphics[width=\linewidth]{figs/GW170823_calibration}
    \caption{GW170823}
\end{figure*}
